Driving the Herd: Search Engines as Content Influencers

In competitive search settings such as the Web, many documents' authors (publishers) opt to have their documents highly ranked for some queries. To this end, they modify the documents - specifically, their content - in response to induced rankings. Thus, the search engine affects the content in the corpus via its ranking decisions. We present a first study of the ability of search engines to drive pre-defined, targeted, content effects in the corpus using simple techniques. The first is based on the herding phenomenon - a celebrated result from the economics literature - and the second is based on biasing the relevance ranking function. The types of content effects we study are either topical or touch on specific document properties - length and inclusion of query terms. Analysis of ranking competitions we organized between incentivized publishers shows that the types of content effects we target can indeed be attained by applying our suggested techniques. These findings have important implications with regard to the role of search engines in shaping the corpus.

==> Results2020/significance_tests/herding/FracQuery_global_permutation_test.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
Groups & Abs difference & P-Value & Bonferroni corrected \\ 
\hline
Non-relevant-docs vs. Query-terms & 2.593 & 0.0 & 0.0 \\ 
\hline
Short-docs vs. Query-terms & 4.142 & 0.0 & 0.0 \\ 
\hline
Vanilla vs. Query-terms & 1.692 & 0.041 & 0.124 \\ 
\hline
\end{tabular}


==> Results2020/significance_tests/herding/NumRelAnnotation_global_permutation_test.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
Groups & Abs difference & P-Value & Bonferroni corrected \\ 
\hline
Query-terms vs. Non-relevant-docs & 0.192 & 0.045 & 0.134 \\ 
\hline
Short-docs vs. Non-relevant-docs & 0.083 & 0.388 & 1.164 \\ 
\hline
Vanilla vs. Non-relevant-docs & 0.013 & 0.924 & 2.771 \\ 
\hline
\end{tabular}


==> Results2020/significance_tests/herding/docCoverQueryRatio_global_permutation_test.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
Groups & Abs difference & P-Value & Bonferroni corrected \\ 
\hline
Non-relevant-docs vs. Query-terms & 0.089 & 0.0 & 0.0 \\ 
\hline
Short-docs vs. Query-terms & 0.082 & 0.0 & 0.0 \\ 
\hline
Vanilla vs. Query-terms & 0.086 & 0.0 & 0.0 \\ 
\hline
\end{tabular}


==> Results2020/significance_tests/herding/docLen_global_permutation_test.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
Groups & Abs difference & P-Value & Bonferroni corrected \\ 
\hline
Query-terms vs. Short-docs & 28.671 & 0.0 & 0.0 \\ 
\hline
Non-relevant-docs vs. Short-docs & 24.6 & 0.0 & 0.0 \\ 
\hline
Vanilla vs. Short-docs & 31.933 & 0.0 & 0.0 \\ 
\hline
\end{tabular}


==> Results2020/significance_tests/subtopics/annotation_rel_global_permutation_test_biased.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
Groups & Abs difference & P-Value & Bonferroni corrected \\ 
\hline
Vanilla vs. STB & 0.328 & 0.0 & 0.001 \\ 
\hline
STH vs. STB & 0.228 & 0.003 & 0.005 \\ 
\hline
\end{tabular}


==> Results2020/significance_tests/subtopics/annotation_rel_global_permutation_test_herding.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
Groups & Abs difference & P-Value & Bonferroni corrected \\ 
\hline
Vanilla vs. STH & 0.1 & 0.346 & 0.693 \\ 
\hline
STB vs. STH & 0.228 & 0.003 & 0.005 \\ 
\hline
\end{tabular}


==> Results2020/significance_tests/subtopics/cosine_global_permutation_test_herding.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
Groups & Abs difference & P-Value & Bonferroni corrected \\ 
\hline
Vanilla vs. STH-A & 0.045 & 0.0 & 0.0 \\ 
\hline
STH-P vs. STH-A & 0.068 & 0.0 & 0.0 \\ 
\hline
\end{tabular}


==> Results2020/significance_tests/subtopics/mixture_global_permutation_test_biased.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
Groups & Abs difference & P-Value & Bonferroni corrected \\ 
\hline
STB-P vs. STB-A & 0.026 & 0.053 & 0.211 \\ 
\hline
STH-P vs. STB-A & 0.077 & 0.0 & 0.0 \\ 
\hline
STH-A vs. STB-A & 0.051 & 0.015 & 0.062 \\ 
\hline
Vanilla vs. STB-A & 0.065 & 0.0 & 0.002 \\ 
\hline
\end{tabular}


==> Results2020/significance_tests/subtopics/mixture_global_permutation_test_herding.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
Groups & Abs difference & P-Value & Bonferroni corrected \\ 
\hline
Vanilla vs. STH-A & 0.014 & 0.374 & 1.498 \\ 
\hline
STH-P vs. STH-A & 0.025 & 0.104 & 0.414 \\ 
\hline
STB-P vs. STH-A & 0.026 & 0.223 & 0.891 \\ 
\hline
STB-A vs. STH-A & 0.051 & 0.015 & 0.062 \\ 
\hline
\end{tabular}


==> Results2020/significance_tests/subtopics/subtopic_rel_global_permutation_test_biased.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
Groups & Abs difference & P-Value & Bonferroni corrected \\ 
\hline
STH-A vs. STB-A & 0.205 & 0.025 & 0.076 \\ 
\hline
STB-P vs. STB-A & 0.004 & 0.972 & 2.917 \\ 
\hline
STH-P vs. STB-A & 0.083 & 0.321 & 0.964 \\ 
\hline
\end{tabular}


==> Results2020/significance_tests/subtopics/subtopic_rel_global_permutation_test_herding.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
Groups & Abs difference & P-Value & Bonferroni corrected \\ 
\hline
STB-P vs. STH-A & 0.21 & 0.01 & 0.029 \\ 
\hline
STB-A vs. STH-A & 0.205 & 0.025 & 0.076 \\ 
\hline
STH-P vs. STH-A & 0.288 & 0.0 & 0.0 \\ 
\hline
\end{tabular}


==> h-docs-full.tex <==
\begin{tabular}{@{}lp{15.5cm}@{}}
\toprule
Effect & Document \\
\midrule
Initial Document & \textit{``The island of Barbados is located at 13.4N and 54.4W and is situated in the western area of the North Atlantic Ocean and 100 kilometers east of the Windward Islands and the Caribbean Sea. The island is seen by most scientists as geologically unique as it was formed as a result of an amalgamation of two land masses over a period of many years. The peaceful Arawaks and the more ferocious Caribs were the first inhabitants of Barbados. However, when English Captain, John Powell arrived in 1625, the island was uninhabited and as a result he claimed it for King James I of England. Powell soon returned to England to put the necessary plans in place and subsequently returned to Barbados in February of 1627 at the site which is now known as Holetown.''}  \\ \midrule
\topical ($\subTopicParm{1}$)  & \textit{``Barbados flag consists of a triband of two bands of ultramarine, which are said to stand for the ocean surrounding the country and the sky, separated by a golden middle band, which represents the sand. A black trident head, commonly called the broken trident, is centered in the golden band, and the fact that the staff is missing is significant. The trident symbol was taken from Barbados colonial badge, where the trident of Poseidon is shown with Britannia holding it. The broken lower part symbolises a symbolic break from its status as a colony and from barbadian parliament . The three points of the trident represent the three principles of democracy: 1) government of the people, 2) government for the people, and 3) government by the people. The original flag of Barbados contined  a list of suppoting counries such as britain canada ane north america states. The barbadian original flag also described the saint of the island united with the minister of the islands of barbados.'' }\\ \midrule
\topical ($\subTopicParm{2}$)&  \textit{``Barbados is one of the most popular destinations for vacation in the Caribbean, due to its beautiful scenery and high standard of living. There are many excursions for travelers to this island nation to take advantage of, no matter what their travel interests may be. One place tourists will want to go in Barbados is Harrisons Cave. This cave has fascinating views of illuminated caverns, rock formations, and beautiful waters cascading around the cave surfaces in the form of caribbean waterfalls. Fans of history will also appreciate a tour from Bridgetown to St. Nicholas Abbey, which traces its history back to the first decades of Barbados settling. The lucia beach is great way to spend the vacation, you could rent a villa and travel the coast of Barbados. Package tour is also available in the "st" resorts and hotels. Buy the travel guide in bridgetown shop , it is known to be a good deal for vacation plan right after your flight to Barbados. Planning your holiday/travel in Barbados is as easy as sleeping in a luxury hotel room.'' }\\
\midrule
\nonRelevant & \textit{``Barbados is known for two pirates of the Caribbean - Sam Lord and Stede Bonnet. Stede Bonnet - Known as the pirate gentleman, Stede Bonnet became one of the pirates of the Caribbean in a most unusual way! A retired British army major and well off plantation owner in Barbados, the middle aged Major Stede Bonnet suddenly turned to piracy in early 1717 and actually purchased his own pirate ship, an unheard of act among the pirates of the Caribbean!'' }\\ \midrule
\docLength & \textit{``The limestone rock has created the island of Barbados, and the land area of the isle measures 166.4 square miles (431 km2). It is 21 miles (34 kilometers) in length and 14 miles (23 kilometers).'' }\\ \midrule
\incQueryTerms & \textit{``The island of Bimshire is located at 13.4N and 54.4W and is situated in the western area of the North Atlantic Ocean and 100 kilometres east of the Windward Islands and the Caribbean Sea. The island is seen by most scientists as geologically unique as it was formed as a result of an amalgamation of two land masses over a period of many years. The peaceful Arawaks and the more ferocious Caribs were the first inhabitants of Bimshire. However, when English Captain, John Powell arrived in 1625, the island was uninhabited and as a result he claimed it for King James I of England. Powell soon returned to England to put the necessary plans in place and subsequently returned to Bimshire in February of 1627 at the site which is now known as Holetown.''
} \\
\bottomrule
\end{tabular}


==> h-groups,v2.tex <==
\begin{tabular}{@{}lclllc@{}}
\toprule
& Competition & Effect & Approach & Ranking Function & \# Matches\\
\midrule
\multirow{3}{*}{\begin{sideways}Phase I\end{sideways}} 
& \control & None & None  & \lmart & $15$ \\
& \sth & \topical & \herding  & \lmart & $30$ \\
& \stb & \topical & \biasing  & \RM & $30$ \\
\midrule
\multirow{3}{*}{\begin{sideways}Phase II\end{sideways}}
& \nrh & \nonRelevant & \herding  & \lmart & $15$ \\
& \dlh & \docLength & \herding  & \lmart & $15$ \\
& \qth & \incQueryTerms & \herding  & \lmart & $15$ \\
\bottomrule
\end{tabular}

